Recent Research Advances on Interactive Machine Learning

Interactive Machine Learning (IML) is an iterative learning process that tightly couples a human with a machine learner, which is widely used by researchers and practitioners to effectively solve a wide variety of real-world application problems. Although recent years have witnessed the proliferation of IML in the field of visual analytics, most recent surveys either focus on a specific area of IML or aim to summarize a visualization field that is too generic for IML. In this paper, we systematically review the recent literature on IML and classify them into a task-oriented taxonomy built by us. We conclude the survey with a discussion of open challenges and research opportunities that we believe are inspiring for future work in IML.

==> LaTeX of JOVI-D-18-00101-local/ack.tex <==
% \begin{acknowledgements}
% The authors are supported by National
% NSF of China (No. XXX). 
% We would like to thank the reviewers for their constructive suggestions to improve the quality of the paper. 
% \end{acknowledgements}

==> LaTeX of JOVI-D-18-00101-local/anomaly.tex <==
\begin{figure*}[!tb]\centering
\includegraphics[width=\linewidth]{fig/AnomalyDetection_sequences}
\caption{TargetVue~\cite{cao2016targetvue}: (a) behavior glyph shows the activities of a user over time; (b) z-glyph shows z-score of features; (c) relation glyph shows relationships of users in online communication systems.}\label{fig:AnomalyDetection_sequences}
\end{figure*}
\subsection{Interactive Anomaly Detection}
% all reference~\cite{bogl2017cycle,cao2016targetvue,xu2017vidx,leite2018eva,lin2017rclens,wilkinson2018visualizing,cao2018voila}

% Anomaly detection refers to the process of detecting objects with unexpected behaviors. 
Interactive anomaly detection refers to the disclosure of anomalies, which are defined as the data with unexpected behaviors~\cite{han2011data}, with human in the process. 
% We summarize the recent literatures about interactive anomaly detection into two categories: anomalous points detection and anomalous sequences detection~\cite{zhao2014fluxflow}. 
We classify the recent literature into two categories: anomalous points detection ~\cite{bogl2017cycle, cao2018voila, leite2018eva, lin2017rclens, wilkinson2018visualizing} and anomalous sequences detection~\cite{cao2016targetvue, xu2017vidx}. 
% % Automatic anomaly detection is extensively studied in machine learning community and widely applied in practice. 
% However, automatic anomaly detection faces two challenges. 
% First, 
% labeled data for training is usually hard to collect because of the rarity nature of abnormal cases and the unclear boundary between abnormal objects and normal ones. 
% \changjian{Besides, 
% the cost of false positive and false negative is so expensive that users would not fully trust in an automatic anomaly detection method.
% For instance, 
% % wrongly marking a normal account as fraud 
% marking a normal transaction as unauthorized one 
% would lead to the loss of customers.} 
% % Cooperating human analyzing ability with automatic anomaly detection 
% To tackle these challenges, interactive anomaly detection methods have been proposed to loop human into the detecting procedure and promote confidence in the detecting results. 
% % Recent interactive anomaly detection methods mainly address three types of data: \changjian{tabular data}, temporal data and spatio-temporal data. 
% % We survey the recent literature and identify that recent interactive anomaly detection methods mainly focus on sequential data. 
% As anomalous patterns is arbitrary and primarily depends on data, we surveyed the recent literature and categorized recent work by data type: event sequential data and spatio-temporal data.  

\subsubsection{Anomalous Points Detection}
% Event sequential data, 
% like financial transaction or user generated content, is the most widely explored data type in interactive anomaly detection. 
% % Basically, anomaly detection of event sequential data can be divided into two parts: 
% Basically, anomaly detection of event sequential data consists of two primary parts: 
% anomalous event detection like unauthorized transaction detection, and anomalous sequential detection like spammer detection in online communication systems. 
% Detecting unexpected events that deviate from historical patterns is the primary goal of anomalous event detection. 
Anomalous points detection refers to the detection of individual points with unexpected behaviors.
For example, Leita et al. propose EVA~\cite{leite2018eva}, a visual analytics system for interactive fraudulent transaction detection.
% \changjian{Instead of visually presenting binary (positive or negative) results to users,} 
% Instead of visually presenting the binary results that objects are anomalies or not to users, 
% Comparing to a binary result determining whether a object is an anomaly, anomalous score is a more informative description. 
% Consequently, 
They employ a profile-based algorithm to characterize customers based on their historical transactions.
To measure the overall anomaly score of an incoming transaction, a scoring system is used to compare the transaction with the profile of its corresponding customer.
Specifically, the overall anomaly score is calculated by summarizing the sub-scores of the transaction, which are visualized in a parallel coordinate plot (Fig.~\ref{fig:AnomalyDetection_points}B) to show their contribution to the overall score.
Exploring the parallel coordinate plot, users can relate each sub-score to the overall score for comparatively analyzing the pattern of an anomalous transaction.
% A scoring system compares each incoming transaction with the corresponding customer's profile and outputs several sub-scores reflecting different aspects of an overall score. 
% and a scores generation algorithm to assign an overall anomalous score to each financial transaction. 
% which is a more informative description than binary one.  
% Scores are more informative descriptions than binary ones. 
% These sub-scores are exhibited via a parallel coordinate plot(Fig.~\ref{fig:AnomalyDetection_points}B) to expose the influences of different aspects on the overall score.
% These sub-scores are ~\jiangl{visualized in} a parallel coordinate plot (Fig.~\ref{fig:AnomalyDetection_points}B) to expose the influences of different aspects on the overall score. 
% Via this visualization with other coordinated visualizations like ranks view, users are able to reason the anomalous transactions in an interactive manner. 
% \jiangl{The parallel coordinate plot is coordinated with other views such as the rank view} to allow users to interactively analyze the anomalous transactions. 
% the reason why a anomalous transaction happens. 
% Coordinated views, like scatter plot and bar chart, support interactive explore transactions and compare accounts. 
% Based on the insights obtained via EVA, users can fine-tune the automatic algorithm for better performance. 
Anomalous points detection are more challenging for streaming spatio-temporal data due to its massive volume and heterogeneity~\cite{cao2018voila} .
% \changjian{The challenges come from two aspects.} 
% The challenges come from two aspects~\cite{cao2018voila}.
% First, spatio-temporal data is massive and heterogeneous and in a streaming format; a real-time method to process such data is demanding. 
% On the other hand, How to visually represent spatio-temporal data with rich context information in a comprehensive manner is also nontrivial. 
% A recent work, Voila~\cite{cao2018voila}, has been proposed to detect anomalous points in streaming spatio-temporal data. 
To address this issue, Cao et al. propose Voila~\cite{cao2018voila}, a visual analytics approach for online detecting anomaly on streaming spatio-temporal data.
Specifically, they formulate the spatio-temporal data as a tensor and decompose it to derive latent representations of region, time and feature.
% They based on tensor decomposition is employed to extract latent representations of region, time and feature.
%has been proposed to detect anomalous points in streaming spatio-temporal data. 
% To support the real-time and online processing of such data, an anomaly detection method based on tensor decomposition is employed to extract latent representations of region, time and feature. 
Thus, the anomalous patterns can be extracted from incoming data by comparing the incrementally updated latent representations to that in history.
They use geographic visualization to show the anomalous patterns, which enables a user to provide feedback such as confirming or rejecting an anomalous pattern, to interactively steer the detection model.
% The anomalous patterns of region and time, which is easier to comprehend by human than raw spatio-temporal data, are exhibited via a map view and a temporal pattern view. 
% Users can confirm anomalous patterns proposed by algorithm or identify hidden ones.
%Anomalous patterns will update in a Bayesian manner with users feedback. 

\subsubsection{Anomalous Sequences Detection}
Anomalous sequences detection is the process of identifying sequences with unexpected behaviors.
% To this end, 
Cao et al.~\cite{cao2016targetvue} propose TargetVue to detect Internet users 
% , which are represented by a series of user generated contents, 
with anomalous behaviors in online communication systems. 
To characterize the behaviors of Internet users, they extract a set of features from multiple perspectives, such as the user post and interaction between users. 
They visualize the characterized behaviors using glyphs (Fig.~\ref{fig:AnomalyDetection_sequences}), which enables a user to detect and reason about the anomalous patterns.
% With such rich-content visual representations, anomalous patterns can be easily detected and reasoned. 
% A time-adaptive local outlier factor algorithm is implemented to detection anomalous users. 
% Users can fine-tune the parameters of algorithm based on the knowledge obtained via several coordinated views. 
% Another interesting type of temporal data is assembly line data.
Another interesting application of anomalous sequences detection is the performance diagnostics of assembly line.
% Assembly line data contains informative logs, like starting time or fault codes, of a part when it is processed by work stations in the assembly line. 
% The logs of a part is called a process. 
% Unlike user generated content data that is well described by multiplicate features, most of assembly line data are timestamps, which gives rise to challenges in both visualization and automatic anomaly detection.
% In an assembly line, one product are processed by work stations along the line and logs like time and states are recorded 
Assembly line data contains a massive amount of logs collected from the product manufacturing process.
% Specifically, as the timestamps are time-dependent, the assembly line data are supposed to be displayed in a neatness, time-ware way. 
To address the diagnostics on assembly line, Xu et al.~\cite{xu2017vidx} propose a visual analytics approach, ViDX, based on adapting the Marey's graph to represent each process as a polyline. 
% , which aggregates normal processes and highlights anomalous ones, to overcome clutter. 
To reduce the visual clutter caused by massive amount of data, ploylines representing normal processes are aggregated as thick bands while anomalous ones are highlighted. 
The timeline of the Marey's graph is the topological sort of the abstract directed acyclic graph representation of assembly line, which facilitates users to trace the product history.
By interactively incorporating user feedback, the user-identified
anomalous processes are propagated to other processes for improving the detection accuracy.
% The first one is quantiles brush, which allows users define a quantiles range. 
% Processes with processing time exceeding this range on any station are regarded as anomaly. 
% The other one requires users' labels of several processes. 
% More anomaly will be detected via a label propagation algorithm. 


% Another interesting work that relative to anomaly detection is RCLens~\cite{lin2017rclens}. 
% RCLens addresses the rare category detection problem. 
% Like anomaly detection, rare category detection detect the minority of data that deviates from the overall structure. 
% However, as anomalies are individual exceptions, a rare category refers to a subset of data with similar structure. 
% As high dimensionality could bring challenge into detecting rare categories, RCLens incorporates a feature distribution view that reveals the variances of features and a novel snapshot glyph that visually summarizes subspace users selected. 
% Given these two visual components, users can interactively explore different subspaces and identify these in which rare categories are well separated. 
% Instances are projected into two-dimensional plane that helps users identify or refine rare category results. 
% Users' feedback will be processed by the LOF-based Rare Category Detection algorithm to promote a better results. 


==> LaTeX of JOVI-D-18-00101-local/conclusion.tex <==
\section{Conclusions}
This paper provides a survey of recent research advances on IML.
We review recent literatures on IML, classify them into a task-oriented taxonomy built by us, and summarize the work focusing on the tasks less discussed by existing surveys, including visual pattern mining, interactive anomaly detection, interactive information retrieval, and visual topic analysis.
%We also discuss research opportunities based on presenting the technical challenges as well as inadequately investigated IML areas that can make IML better satisfy the requirements of real-world applications.
We also discuss research opportunities for future work on IML. 

==> LaTeX of JOVI-D-18-00101-local/discussion.tex <==
\section{Research Challenges and Opportunities}
\label{sec:cha_oppt}
Although IML benefits many real-world applications by looping human into the learning process, it still faces several research challenges. 
Here, we highlight the major research challenges, which may pave the way for further research opportunities.
\\

\noindent\textbf{Wide and easy adoption of machine learning techniques}.
Although machine learning provides benefits for almost each industry, its adoption faces several barriers.
First, many learning models perform the same functions (e.g., classification), however, business practitioners usually do not have enough knowledge to decide which one to use. 
As a consequence, it is necessary to study interactive model recommendation, which aims to select the appropriate learning models for a given task and requirement.  
One key challenge here is to leverage interactive visualization to illustrate how the automatic machine learning techniques find the best possible modeling technique for a particular problem. 
Second, parameter settings generally have significant influence on the performance of the learning model.
As a result, a fine tuning of model parameters is required for most of the learning models to obtain satisfactory results.
Accordingly, one challenge is how to systematically explore the multi-dimensional parameter space to greatly reduce the search space of model parameters.
\\

\noindent\textbf{Scalability}.
The size of the model as well as the volume of data are ever-growing in the era of big data.
Visualizing models with complex structures and large numbers of components is challenging, 
especially when the models handle tens of thousands of data items. 
For example, if ResNet-101 is utilized to train a model on a dataset with millions of images and hundreds of categories, it is usually difficult to develop an appropriate visual summarization or abstraction to support model analysis and prediction understanding tasks.
Accordingly, visualization researchers desire to design and develop scalable visualizations to simultaneously convey the model structure, prediction results, and the raw data, as well as to link them together, for a comprehensive analysis of the learning process and results.  
\\

\noindent\textbf{Explainability for data scientists and practitioners}. 
Most existing work focuses on the understanding and analysis of the training process, where the target users are machine learning experts~\cite{liu2017towards_survey}. 
Such type of explainability is very useful for machine learning experts to build robust and high performance learning models. 
However, in real-world settings, data scientists and practitioners also require the explainability of machine learning models to build AI-related applications that business experts can rely on for making informed decisions.
The major obstacle is the trade-off between predictive performance and explainability. 
Typically, decision-tree-based methods can be easily understood by users who are not experts in machine learning. 
On the other hand, ensemble methods such as deep learning models, random forests or boosting trees built upon decisions trees usually achieve better performance.
However, the complexity of the ensemble models usually decreases explainability.
As a result, one interesting venue is to study how to leverage the self-explainable machine learning models such as decision trees to illustrate the working mechanism and predictions of the ensemble models. 
This enables the practitioners to better understand the model predictions and select the appropriate models and parameters for their tasks. 
\\

\noindent\textbf{Monitoring and debugging the online training/testing process of machine learning models}.
In recent two years, there are some initial efforts in debugging offline training process after the training is finished~\cite{choo2018visual}, which already shows the prominence in helping machine learning experts identify the root cause of failure, as well as improve and refine the learning model. 
However, in real-world applications, the training process of many machine learning models is very time-consuming, which can sometimes take up from hours to days~\cite{pu2016variational}.
It is a painful experience to train such models since the training relies on a large number of trial-and-error experiments~\cite{liu2017towards_survey}.
Thus, it is desired to monitor the online training process and find the potential issue(s) that may lead to an unsatisfactory training process.  
One possible solution is to leverage progressive visual analytics techniques to integrate experts into the analysis loop. 
To achieve this, machine learning models are expected to produce semantically meaningful partial results in the training/testing process. 
By leveraging interactive visualizations, experts explore and analyze the system generated partial results, compare newly incoming results with previous ones, a well as perform analysis without having to wait for the entire training process to be completed. 
\\

\noindent\textbf{Improving data quality}.
In machine learning, data and model are equally important.
Thus, data quality is also very important in machine-learning-related applications.
However, during the data collection stage, some inaccurate or error data can be included, which usually affects the further usage of data (e.g. lower the accuracy of the learning models). 
For example, crowdsourcing is a popular way to acquire labeled data. 
Due to individual differences among workers in terms of background, knowledge, and expertise, crowdsourced annotations may be noisy and poor in quality and usually require additional validation~\cite{liu2018interactive}.
As a result, one key issue on preparing and preprocessing data is to ensure the quality and usability of data.
To improve data quality, it is necessary to leveraging interactive visualization for better illustrating the data distribution, identifying potential errors, and minimizing the workload of domain experts who verify the data. 
For example, interactive visualization can be leveraged to tightly combine user-guided methods with system-guided methods during the verification process.



% \textbf{Quality of DR}
% \begin{itemize}
% \item Many IML approach rely on inspecting the DR results of the high-d data or model variables, however, the patterns observed in DR results, may be misleading, e.g., density in a t-SNE plot is known to not faithfully reveal the high-D data density. 
% \item Hence, visualizing DR errors (often w.r.t each data point) for IML applications is important to validating the patterns observed. 
% \item However, visual channels that encodes errors of the DR may conflict with that encodes other information regarding cluster memberships, class, prediction accuracy etc., this may pose design challenges to researchers.
% \item It remains an open question regarding how to choose proper measures to compute errors of DR, and how to translate these errors to semantic meaning for interpreting the DR results ?
% \end{itemize}
% \textbf{User-guided model steering}
% \begin{itemize}
% \item It is important but challenging to present guidance such as interestingness metrics, to recommend interesting data / features / model variables or parameter to users for model steering~\cite{bernard2018comparing}. It would reduce the vast search space of users and save exploration efforts.
% \end{itemize}
% \textbf{Uncertainty}
% \begin{itemize}
% \item uncertainty can be introduced in stages of machine learning  (e.g., data collection, algorithm design, model building)~\cite{wang2016learning}, and stages of visualization process (e.g., DR)~\cite{liu2014survey}.
% \item quantifying and presenting uncertainty to users are important to building trust and informing decision-making~\cite{sacha2016role, correa2009framework, wu2010opinionseer}
% \item How to track the provenance/source of uncertainty ?
% \item How to measure the uncertainties introduced in each stage ?
% \item How to model the interactions of different types of uncertainties~\cite{liu2017towards_survey} ?
% \end{itemize}

==> LaTeX of JOVI-D-18-00101-local/introduction.tex <==
\section{Introduction}
% In the big data era, the explosion of the volume, dimension and variety of data poses challenges for researchers and practitioners to perform sensemaking and analytical reasoning.
% To tackle the challenges, machine learning community embraces computational power of machines and presents algorithmic methods such as statistical modeling to automatically find the intricate structures of the data,https://v2.overleaf.com/project/5b5c244cee619114ee7108b8
% while visualization community harness perceptual power of humans and develops a suite of visualization tools to empower humans to visually explore the data and perceive the patterns.
% However, though automated models from machine learning community perform well for moderate tasks, they are not satisfactory and even fail for complex scenarios where the data is quite noisy or contains adversarial samples or is not distributed as expected by the model.
% %Furthermore, the ever increasing complexity of machine learning models renders it hard to interpret, the highly complex models such as deep neural network are regarded as "black-box", and there is no obvious method to diagnose and refine the model when it does not achieve satisfactory performance.
% For visualization tools, humans can perfectly detect patterns from a small scale data, however, the scalability is poor because the vision system of humans is limited to 2D/3D and humans are easily overwhelmed by the overdraw when the amount of data is large. 
% Hence, it is almost impossible for humans alone to explore such large amount of high-dimensional data, let alone find the patterns of the data.

% Thus, it would be beneficial to tackling the analytical task if the cognitive ability of humans and the computational ability of machines could be combined together.
% Following this line, Interactive Machine Learning (IML), the learning process of machines with humans in the loop~\cite{amershi2014power}, is coined.
% The typical IML workflow includes two steps in each iteration. First, the intermediate results of the model as well as the data is visually presented to the user, the user explores the visualization results, draw understandings and insights about the data and the model, then input feedback to the model.
% Second,  the model is incrementally updated by integrating the human input.
% Hence, IML enables the model to be interactively steered by humans and it would be more advantageous than the traditional machine learning paradigm where the learning is fully automatic and no human knowledge is available.
% %to add
% %In particular, the learner iteratively incorporates input from a human, incrementally integrates the input into the learning cycle, and then presents the new output to the human for another round of iteration.

% Due to the tight coupling of human intelligence to machines computational ability, IML has been widely used by researchers and practitioners to effectively solve real-world application problems, such as predictive business analytics, traffic pattern mining and high-dimensional biomedical data exploration.
% % However, there are still open challenges for developing effective IML pipelines.
% However, there are still open challenges in IML research.
% For example, the ever increasing complexity of machine learning models renders them hard to interpret to humans, thereby hampering the process of diagnosing and refining the model.
% Further, there is little efforts on understanding the inner working mechanisms of IML or systematically exploring the IML research for deriving insights from this field and presenting future research directions. 


% To address this challenge, we present a comprehensive analysis of recent advances on interactive machine learning by systematically surveying the recent literature in visualization community that focus on IML.
% Specifically, we first provide an overview of current research scope and outline the research trend.
% Then we build a task-oriented taxonomy (Table~\ref{table:tasktaxonomy}) that categorizes the IML research by the overarching task.
% Each task is exemplified by representative work. 
% We also elucidate the interplay between machine learning and visualization to foster a better understanding of the inner working mechanisms of IML and point out the pitfalls in developing sensible IML systems. 
% Referring to our paper, IML researchers and practitioners could be guided towards more effectively and efficiently applying IML to solve real-world problems.
% We conclude the paper by presenting open challenges and research opportunities which we believe are inspiring for future work in IML.
% Machine learning is very powerful and useful for recognizing patterns and making prediction on data.
% It has been applied to a wide variety of domains such as information retrieval, computer vision, pattern recognition, and healthcare.
Although machine learning has gained remarkable attention in many fields including information retrieval, computer vision, pattern recognition and data mining.
%Despite its success, machine learning 
It is often criticized for its ``black box'' learning, complicated parameter tuning, and lack of human knowledge in the problem solving processing. 
%human interaction is still needed to warrant a high-quality model.
%For example, a machine learning model may incur uncertainties that need to be tackled by a human~\cite{liu2016uncertainty, liu2017improving}, 
%or extract uninteresting patterns that need to be manually~\cite{liu2017towards,liu2014survey,liu2017towards_survey}. %filtered~\cite{chen2018sequence, guo2018eventthread}.
%In light of this, 
To tackle these issues, interactive machine learning (IML) is emerging as a promising field in visual analytics~\cite{fails2003interactive,liu2017improving,liu2017towards}.
It tightly couples human input with machines in the learning process.
For example, IML can facilitate the performance improvement of machine learning models with the help of human knowledge through rich interactions~\cite{liu2016uncertainty, wang2016topicpanorama, wu2018m3}.
%IML is an iterative learning process that tightly couples a human with a machine learner (i.e., a machine learning model).
% In particular, the learner iteratively incorporates input from a human, incrementally integrates the input into the learning cycle, and then presents the new output to the human for another round of iteration.
% Due to the organic combination of the human intelligence and the computational ability of machines, IML is more advantageous than the automatic learning.
% Hence, IML is widely used to solve real-world application problems, such as mobility pattern mining~\cite{chen2016interactive} and high-dimensional data exploration~\cite{pezzotti2017approximated}.
The typical IML workflow includes two steps in each iteration. 
First, the intermediate results of the model as well as the data is visually presented to the user, the user explores the visualization results, draw understandings and insights about the data and the model, then input feedback to the model. 
Second, the model is incrementally updated by integrating the human input.
Hence, IML enables machine learning models to be interactively steered by humans and is more advantageous for the tasks where human knowledge is needed in the analysis process. 

% Though recent years have seen the surge of IML, there are little efforts made to summarize the body of IML work done over the past few years.
Recent years have seen the surge of IML. 
However, most existing surveys either focus on a specific area of IML, including interactive dimensionality reduction~\cite{sacha2017visual}, 
interactive model analysis~\cite{liu2017towards_survey}, visual social data analytics~\cite{wu2016survey}, and predictive visual analytics~\cite{lu2017state}, or aim to summarize the visualization field that is too generic for IML, e.g., information visualization~\cite{liu2014survey, lu2017frontier}.
The most relevant work to ours is the recent survey by Endert et al.~\cite{endert2017state}, they reviewed visual analytics approaches that integrate machine learning models, with a focus on classification, clustering, regression and dimensionality reduction. 
We elaborate on tasks that are less covered by these existing surveys, such as interactive information retrieval and visual pattern mining.

In this paper, we systematically review recent literature on IML and classify them into a task-oriented taxonomy (Table~\ref{table:tasktaxonomy}) built by us.
% For each IML task, we summarize the typical approaches, present the connection of them, and discuss their pros and cons.
We summarize the recent approaches for IML tasks and also point out open challenges and research opportunities that we believe are inspiring for future work in IML.
%The purpose of this survey is threefold.
%First, for newcomers to IML, our paper helps them gain an overview of the field and find the topic(s) of interest.
%Second, referring to our comparison of approaches to tackling each IML task, IML practitioners could be guided on selecting the most suited approaches to address their tasks at hand.
%Third, for IML researchers, we believe they could sense research topics that are not adequately studied and need further investigation.
The purpose of this survey is to provide an overview of the field and help researchers find research topics that are not adequately studied and need further investigation.

% The rest of the paper is organized as follows.
% In Section~\ref{sec:overview}, we provide an overview of the IML research.
% Section~\ref{sec:tasks} elaborates on the approaches to tackling the IML tasks.
% We conclude the paper in Section~\ref{sec:cha_oppt}, which presents challenges and opportunities for future IML studies.

==> LaTeX of JOVI-D-18-00101-local/others.tex <==
\subsection{Discussion on Other Tasks}\label{sec:discuss_others}
\noindent\textbf{Visual cluster analysis}. \jiangl{We refer to visual cluster analysis as the task of interactively partitioning instances to multiple groups based on their similarities.
It uncovers grouping patterns in the data and stands as a fundamental approach for visually aggregating or summarizing the data.
Thus, visual cluster analysis has been applied to many data-driven applications such as weather ensemble forecast~\cite{kumpf2018visualizing} and air traffic optimization~\cite{andrienko2018clustering}.
Recent work mainly focuses on cluster-based exploratory data analysis~\cite{andrienko2018clustering, badam2017steering, heimerl2016citerivers, sacha2018somflow, wu2017mobiseg, wu2017streamexplorer}, comparative clustering analysis~\cite{jarema2015comparative, kumpf2018visualizing, kwon2018clustervision, zhang2016visualizing}, and bi-cluster analysis~\cite{sun2016biset, watanabe2015biclustering, wu2017making, wu2015interactive, zhao2018bidots}.}
\\

\noindent\textbf{Interactive dimensionality reduction}. \jiangl{Recent years have seen a plethora of work on interactive dimensionality reduction for visually analyzing high-dimensional data.
They mainly address subspace analysis~\cite{jackle2017pattern, liu2015visual, wang2018subspace, wang2017linear} and progressive high-dimensional data exploration~\cite{pezzotti2016hierarchical, pezzotti2017approximated, turkay2017designing}.
One important component in human-centered dimensionality reduction is the interaction.
They can be classified into three categories: manipulating data points (e.g., dragging and dropping instances to define constraints), interacting with features (e.g., tuning weights of dimensions) and modifying model variables (e.g., rotating projection bases).
For more details about the interaction paradigm, we refer readers to existing surveys such as~\cite{endert2017state, sacha2017visual} that have comprehensively categorized and analyzed the interaction intent and scenarios.}
\\

\noindent\textbf{Interactive classification}. \jiangl{Recently, interactive classification has been applied to a wide variety of applications including drug relation analysis~\cite{verma2017drugpathseeker}, urban planning~\cite{yu2015iviztrans}, relationship exploration in multi-party conversations~\cite{el2017nerex} and user demographic analysis~\cite{dou2015demographicvis}.
The quality of labels, features and parameter tuning are important factors to building a high-performance classifier.
Hence, based on which factor the interactive classification focuses on, we classify recent work into three categories: interactive labeling, interactive feature engineering and parameter space analysis.
The work on interactive labeling mainly loop humans in removing annotation noise and inspecting the labels of the most uncertain instances~\cite{bernard2018comparing}.
For interactive feature engineering, recent work focuses on visually constructing discriminative features~\cite{brooks2015featureinsight} and facilitating users to understand the correlation between features and classes~\cite{dou2015demographicvis}.
Recent work related to parameter space analysis mainly propose interactive visualization for users to navigate and explore parameter space~\cite{rohlig2015supporting} and provide visual cues to users for understanding the influence of the parameters~\cite{muhlbacher2018treepod}, such as the sensitivity of the classification results to parameters.}
\\

\noindent\textbf{Interactive regression}.
\jiangl{While interactive classification deals with categorical labels, interactive regression refers to the prediction of continuous values by modeling the relations between independent and dependent variables.
Recent work applies interactive regression to many real-world problems such as disease risk factor analysis~\cite{klemm20163d}, causality reasoning~\cite{wang2016visual} and prediction of scientific emulation~\cite{bryan2015integrating}.
They can be categorized into interactive correlation analysis~\cite{klemm20163d, shao2017interactive, wang2016visual, zhang2016visual, zhang2015visual} and interactive numerical prediction~\cite{bryan2015integrating, buchmuller2015visual, lowe2016visual}.
Interactive correlation analysis focuses on visually mining relationships among variables of data, based on the regression models.
Users can inject their domain knowledge to the regression models by interacting with the visual representation of the variable correlations~\cite{klemm20163d, zhang2015visual}, typically a graph representation such as matrices or node-link diagrams.
For interactive numerical prediction, recent work mainly visualizes the quality of regression (e.g., error residuals) to guide users to interactively explore prediction results, select models and tune parameters.
For a detailed description of the pipeline, interaction and tasks of interactive regression, we refer readers to Lu et al.'s recent survey on predictive visual analytics~\cite{lu2017state}.}
\\

\noindent\textbf{Interactive model analysis}. \jiangl{Understanding machine learning models and interpreting their behaviors are important to an informed user interaction in IML applications~\cite{krause2017workflow}.
Hence, interactive model analysis (e.g., understanding and diagnosing models) has attracted recent research attention.
Researchers mainly propose interactive visualizations to facilitate users to reason about the working mechanism of models (e.g., interaction between neurons in deep neural network) and diagnose an unsatisfactory learning process (e.g., convergence failure)~\cite{liu2017towards_survey, liu2018analyzing_noise}.
Liu et al.~\cite{liu2017towards_survey} elaborated on interactive model analysis in a recent survey and we follow their method to categorize the related work.
More recently, Choo and Liu~\cite{choo2018visual} and Hohman et al.~\cite{hohman2018visual} systematically reviewed and summarized visual analytics systems with a focus on the analysis of deep learning.
Readers can find detailed information about interactive model analysis in those previous surveys.}

==> LaTeX of JOVI-D-18-00101-local/overview.tex <==
\section{Overview and Scope}
\label{sec:overview}
In this survey, we reviewed existing work on IML from visual analytics community, where interactive visualizations empower users to iteratively steer machine learning models.
We reviewed related papers from 2015 to 2018 in the following journals or conferences: IEEE TVCG, IEEE VAST, IEEE InfoVis, EuroVis, and IEEE PacificVis.
% To collect the papers relevant to IML, we adopted a two-step manual selection strategy.
% First, we exhaustively checked the titles and abstracts from the proceedings of the conferences (or IEEE TVCG)  to find candidate papers.
% Second, for the uncertain candidate papers, we reviewed their full texts to determine their relevance to IML.
To collect the IML papers, we exhaustively checked the titles and abstracts from the proceedings of the conferences (or IEEE TVCG) to find candidates.
Then, we browsed the full texts of uncertain candidates to finalize the selection.
\jiangl{As a result, a total of 99 papers are selected for review.}

% As shown in Table~\ref{table:tasktaxonomy}, we built a taxonomy to classify the related papers based on their analysis tasks.
% The taxonomy have 9 tasks including classical tasks such as ``clustering'', ``dimensionality reduction,'' and recent emerging tasks such as ``model understanding.''
% The ``clustering'' captures the largest number of the papers due to prevalence of data analysis based on interactive clustering.
% As high-dimensional data is ubiquitous in practical applications, we see  a good number of papers fall into the task ``dimensionality reduction''.
% It is noteworthy that ``model understanding'' also capture a fair amount of papers.
% This is due to the proliferation of recent work on opening the ``black-box'' of deep learning.
As shown in Table~\ref{table:tasktaxonomy}, we build a taxonomy to classify the related papers based on their analysis tasks.
\jiangl{The first-level tasks are first initialized to the ones defined by existing IML surveys on specific areas, e.g., interactive dimensionality reduction  identified by Sacha et al.~\cite{sacha2017visual}.
% We then expand them to accommodate papers not pertinent to the initial IML tasks defined by Sacha et al.
We then expand them to accommodate papers not pertinent to those initial IML tasks.
For example, we find the visual analytics work on detecting anomaly does not fall into the scope of the initial tasks and thus add ``interactive anomaly detection'' to the first-level IML tasks.}
% The first-level tasks are selected based on the common machine learning tasks (e.g., clustering) supported by the visual analytics systems.}
In total, it results in 9 tasks including classical ones such as ``visual cluster analysis,'' ``interactive dimensionality reduction,'' and recent emerging tasks such as ``interactive model analysis.''
The ``visual cluster analysis'' captures the largest number of the papers \jiangl{(20)} due to the prevalence of data analysis based on interactive clustering.
As high-dimensional data is ubiquitous in practical applications, we see a good number of papers \jiangl{(16)} fall into the task ``interactive dimensionality reduction''.
It is noteworthy that ``interactive model analysis'' also capture a fair amount of papers \jiangl{(14)}.
This is due to the proliferation of recent work on opening the ``black-box'' of deep learning.
%To keep the taxonomy concise, for a good readability, we merge some ranking and searching to info retrie.
\jiangl{It is worth noting that while most papers can be clearly placed to one analysis task (e.g., ``interactive regression''), 
some papers are related to more than one tasks (e.g., ``interactive dimensionality reduction'' and ``visual topic analysis'' often co-occur within one paper).
For the latter cases, we classify papers to the IML tasks that most emphasizes the roles of humans in their particular scenarios.}
\jiangl{To build the taxonomy in the second-level, we follow the previous task taxonomies that cover our first-level tasks.
For example, we refer to ~\cite{liu2018bridging} for categorizing work on ``visual topic analysis'' into ``flat topic analysis,''``hierarchical topic analysis'' and ``topic evolution analysis.''
For the first-level tasks not covered or not being further classified by the previous work, we categorize the related papers based on their focused aspects of a particular first-level task,  e.g., ``visual pattern mining'' is split into ``exploratory event analysis'' and ``mobility pattern analysis.''}

Existing surveys have reviewed related work on part of these tasks.
For example, ``visual cluster analysis,'' ``interactive classification'' and ``interactive regression'' are discussed in~\cite{endert2017state}, ``interactive dimensionality reduction'' is elaborated in~\cite{sacha2017visual}, and ``interactive model analysis'' is presented in~\cite{choo2018visual, hohman2018visual, liu2018visual}.
We focus on tasks less covered by the existing surveys, such as ``interactive information retrieval.''
% Specifically, we summarize work related to the following tasks: ``interactive information retrieval,'' ``visual topic analysis,'' ``visual pattern mining,'' and ``interactive anomaly detection.'

==> LaTeX of JOVI-D-18-00101-local/pattern.tex <==
\begin{figure*}[!tb]
\centering
    \begin{subfigure}{0.53\textwidth}
          \includegraphics[width=\textwidth]{fig/sequnce_clickstream_border}
    \caption{}\label{fig:sequence_clickstream}
    \end{subfigure}\hspace{8mm}%\hfill
\centering
    \begin{subfigure}{0.38\textwidth}          \includegraphics[width=\textwidth]{fig/sequnce_coreflow_border}
    \caption{}\label{fig:sequence_coreflow}
	\end{subfigure}
    \caption{Examples of visual pattern mining for exploratory event analysis: (a) The level-of-detail visualizations of web clickstreams~\cite{liu2017patterns}: the patterns and segments are visualized using a funnel metaphor (context and pattern view), with their details such as sequences and events shown in an icicle-like plot (sequence view);
(b) CoreFlow~\cite{liu2017coreflow}: the branching pattern is visualized in a node-link diagram with an icicle plot as its background to indicate the length and amount of event sequences.}
\end{figure*}
\subsection{Visual Pattern Mining}
% \begin{figure}[!tb]\centering
% \includegraphics[width=\linewidth]{fig/sequnce_clickstream}
% \caption{~\cite{}. }\label{fig:sequnce_clickstream}
% \end{figure}
% \begin{figure}[!tb]\centering
% \includegraphics[width=0.8\linewidth]{fig/sequnce_coreflow}
% \caption{~\cite{}. }\label{fig:sequnce_coreflow}
% \end{figure}
% Pattern mining generally refers to extracting meaningful patterns from the data. 
% It is a universal task for knowledge discovery, especially for gaining insights from sequential data, such as medical health records and traffic trajectories. 
% Taking medical health records as an example, if we discover the pattern of a frequent co-occurrence of a disease with a symptom, it may indicate their significant correlation. 
% Algorithmic approaches are widely used to extract patterns from the data, however, they may not suffice for effectively solving real-world problems. 
% The reasons are twofold. 
% First, algorithmic approaches have no guarantee to produce salient patterns~\cite{guo2018eventthread}, it is likely to generate redundant or semantically meaningless patterns~\cite{liu2017coreflow}. 
% For most cases, we however have no ground truth to validate the mined patterns. 
% Hence, it is necessary to further explore the semantics of the results and accordingly adjust the model parameters to tune the unsatisfactory results. 
% Second, the complexity of the data such as heterogeneity and noise would exacerbate the problem, because the model would incur high uncertainties that need to be resolved by humans~\cite{guo2018eventthread, chen2018sequence, liu2017patterns, liu2017coreflow}. 
% To tackle the above challenges, the recent years have seen a surge of interactive approaches that loops human into the pattern mining procedure. 

% Comprehensively surveying the recent literature, we spot that they mainly address sequential data. 
% Specifically, they fall into two categories: event sequential data~\cite{guo2018eventthread, chen2018sequence, liu2017patterns, liu2017coreflow} and geospatial movement data~\cite{chen2016interactive, di2016allaboard, krueger2015semantic, poco2015exploring}. 
% We also identify two key stages in interactive pattern mining, i.e., data preprocessing and pattern extraction. 
% Each stage requires human efforts and different applications put emphasis of humans on different stages. 
% For applications on event data, they emphasize humans' role in steering the pattern extraction process (tackling the first challenge). 
% This is due to that they aim to capture interesting and meaningful frequent events to support a more informed decision making, and prune the redundant or meaningless patterns. 
% For applications that focus on the geo-spatial movement data, humans are mostly involved in interactive preprocessing the movement data (tackling the second challenge). 
% This is because the geo-spatial movement data is typically more noisy and heterogeneous. 
% To be more specific, the data contains high uncertainties due to the imprecision of spatial-temporal measurement and it is often enriched with secondary dataset, such as POIs, which increases its complexity. 
% Below we present representative work that exemplify interactive pattern mining from the above two perspectives. 

% For steering the pattern extraction, the key idea is to integrate the semantics cognitive ability of humans into the mining process. 
% Humans can steer the mining process in either a direct or an indirect manner. 
% The direct interaction would be visually modifying the machine-generated results. 
% For example, Liu et al.~\cite{liu2017patterns} employs VMSP algorithm~\cite{fournier2014vmsp} to mine maximal sequential patterns from clickstream data. 
% It empowers users to visually filter out irrelevant sequences and segment the mined sequence patterns. 
% Users could also perform further mining on each segment of the sequence pattern (hierarchical mining). 
% By doing so, the user-driven hierarchical mining could reveal more hidden patterns in the segments, which would otherwise be difficult to discover by machines. 
% Along the same line, Guo et al.~\cite{guo2018eventthread} uses tensor decomposition to derive latent threads (the summarization of sequences) from event data. 
% They allow users to specify the clustering threshold for interactively aggregating semantically similar threads. 
% Integrating human knowledge, the semantically similar threads are grouped together and it leads to a more compact visual summarization of event sequences. 
% It is noteworthy that allowing humans to inspect the semantics of extracted patterns is no easy task, 
% we need level-of-detail interactive visualization to enable an intuitive exploration. 
% Thus, a typical visualization design would be summarizing the sequences for an overview, then visualizing the detailed contexts on user demand~\cite{guo2018eventthread, chen2018sequence, liu2017patterns}. 
% Compared with direct manipulation on mining results, indirect manipulations are more flexible. 
% It enables users to semantically interact with the model by defining interesting or important objects (e.g., event) that the machine-generated patterns are supposed to contain. 
% Following this line, Liu et al.~\cite{liu2017coreflow} allows users to input interesting events to the back-end mining algorithms. 
% Consequently, the back-end algorithms would assign high-priority to the interesting events to guarantee its appearance in the pattern. 
% As not all interesting events are frequent in the dataset, it would otherwise be ignored by the mining algorithms since the pattern mining model generally only discover frequent patterns. 

% For interactive data preprocessing, the relevant work mainly focus on tackling the uncertainties of the movement data that is used for the subsequent pattern extraction. 
% We introduce two representative work that address this problem by human-in-the-loop models. 
% The very first work is presented by Kruger et al.~\cite{krueger2015semantic}. 
% They aim to reveal the semantics underlying movement patterns. 
% To achieve this, they enrich the movement data with POIs obtained from social media. 
% However, due to the imprecision of the measurement on time and space, there is noticeable uncertainty on associating a POI to a geographic position in movement data. 
% To address this, they loop users in the process of categorizing the POI of geographic positions. 
% Specifically, uses can explore the geo-spatial contexts of a given position and change the category of the POI if he disagree with the inferred results from decision model. 
% Consequently, the decision uncertainty on assigning POI to positions can be greatly reduced. 
% Numerical experiments also show the precision of the POI categorization is improved by incorporating human knowledge. 
% Compared with addressing uncertainty of POI assignment in ~\cite{krueger2015semantic}, Chen et al.~\cite{chen2016interactive} aim to tackle the uncertainty of movement data \textit{per se}. 
% They collect a large amount of geo-tagged social media data, then distill movements using the geo-tags. 
% However, the movements distilled from social media are quite noisy and even erroneous. 
% It thus requires efforts on cleaning the movements to warrant a high-quality pattern extraction. 
% To this end, they employ the Gaussian mixtures to directly model the uncertainty of movements and 
% perform a user-driven filtering to obtain reliable data for subsequent pattern extraction. 
% To be specific, users can interactively tune the number of clusters used in fitting Gaussian mixtures. 
% It is useful when the cluster number is either too high so an inherent movement cluster is split or too low so distinct movement clusters get merged. 
% Gaussian mixtures would then induce confidence interval for each cluster and users can directly change the confidence interval according to his knowledge on the semantic meaning of the cluster. 
% The confidence interval are used to filter the movements that are modeled with low confidence. 
% In this manner, most of the low confidence data (typically outliers and error records) are removed and the uncertainty of the movements are reduced.
Visual pattern mining is widely used to interactively discover latent patterns for exploratory correlation or association analysis~\cite{liu2017coreflow,lu2016exploring,poco2015exploring,wen2010mining,yan2018visual}.
%It is a universal task for knowledge discovery, especially for gaining insights from sequential data, such as medical health records and traffic trajectories.
%Taking medical health records as an example, the user may want to discover the pattern of a frequent co-occurrence of a disease with a symptom.
Recent work on visual pattern mining focuses on effectively tackling data-driven tasks including understanding user travel patterns from social media~\cite{chen2016interactive}, analyzing customer behaviors from web clickstreams~\cite{liu2017coreflow, liu2017patterns} and exploring traffic dynamics to improve urban infrastructure~\cite{poco2015exploring}.
%Recently, sequential patterns have attracted the most attention from researchers.
They fall into two categories: exploratory event analysis~\cite{chen2018sequence, guo2018eventthread, liu2017coreflow, liu2017patterns} and mobility pattern analysis~\cite{chen2016interactive, di2016allaboard, krueger2015semantic, poco2015exploring}.
\subsubsection{Exploratory Event Analysis}
Event sequences, i.e., a collection of series that each represents timestamped event occurrences~\cite{chen2018sequence, guo2018eventthread}, can model many real-world data such as user interaction log, machine alert messages and vehicle maintenance records.
Exploratory event analysis mainly focuses on discovering the overall sequential patterns as well as investigating relationship (e.g., causality) between individual events.
Recent work can be classified into two categories: frequency-based~\cite{ liu2017coreflow, liu2017patterns} and clustering-based~\cite{chen2018sequence, guo2018eventthread}.

For frequency-based approaches, frequent pattern mining algorithms are often adopted to extract sub-sequences that frequently occur in the data.
% For example, Liu et al.~\cite{liu2017patterns} a VMSP algorithm~\cite{fournier2014vmsp} to mine maximal sequential patterns from web clickstreams for understanding the shared browsing path of customers.
For example, Liu et al.~\cite{liu2017patterns} adopt a frequency-based algorithm to mine maximal sequential patterns from web clickstreams for understanding the shared browsing path of customers.
%prune them using Jaccard index.
% The mined patterns along with their supporting sequences and events are presented in the level-of-detail visualizations (Fig.~\ref{fig:sequence_clickstream}) to enable an exploratory analysis.
To enable a visual exploration, the mined patterns along with their supporting sequences and events are visualized in a level-of-detail manner, based on a funnel visual metaphor and an icicle-like plot (Fig.~\ref{fig:sequence_clickstream}).
%as well as their semantic information 
%Besides basic interactions such as aligning events, 
Rich interactions are provided to facilitate the exploration, such as aligning events for contextual comparison, and drilling down in a selected pattern segment to disclose its finer-level structures.
%Users can perform further mining on a selected pattern segment to reveal the hidden patterns inside it.
Noticing that the traditional frequency-based approach does not scale to a large-scale dataset and the relationships between the mined patterns remain unclear, 
Liu et al.~\cite{liu2017coreflow} later propose a novel rank-divide-trim algorithm to extract a branching pattern from the event sequences.
The branching pattern is more interpretable to users since it reveals the relationships of frequent patterns in a unified view.
To present the branching pattern, the icicle plot and node-link diagrams are combined to visualize its tree structure as well as the statistics associated with the branches (Fig.~\ref{fig:sequence_coreflow}).
To capture users' interests in specific events, they allow users to define high priority events to inform the mining algorithm to guarantee their appearance in the  pattern. 

For clustering-based approaches, researchers mainly use sequence clustering algorithms to summarize the data for pattern analysis.
For example, Guo et al.~\cite{guo2018eventthread} formulate the event sequences as a three-way tensor, the dimensions of which correspond to entity, stage, event, respectively.
Based on the tensor decomposition, they cluster event sequences to threads that each represent a latent sequential pattern.
The threads are visualized using a line map visual metaphor, and can be interactively grouped by users to reveal the temporal evolution of patterns, such as merging and splitting.
Chen et al.~\cite{chen2018sequence} propose an information-theoretic approach for summarizing the event sequences.
Specifically, they follow the minimum description length principle~\cite{grunwald2007minimum} to find a summarization that balances the conciseness and the information loss.
Based on this approach, they group the data to a set of sequential patterns that stand as a summarization of data.
Due to the lossy nature of the summarization, 
the correction needed to recover the data from the summarization is visualized along with the patterns for a more faithful data representation. 
% \begin{figure}
% \begin{minipage}[t]{0.5\textwidth}
% \centering
% \includegraphics[width=\textwidth]{fig/move_enrich_POI_crop}
% \caption{aaa}
% \end{minipage}
% \begin{minipage}[t]{0.5\textwidth}
% \centering
% \includegraphics[width=\textwidth]{fig/move_enrich_POI_crop}
% \caption{bbb}
% \end{minipage}
% \end{figure}
\begin{figure}[!tb]\centering
\includegraphics[width=0.90\linewidth]{fig/move_enrich_POI_crop}
\caption{Movement patterns semantically enriched with POIs~\cite{krueger2015semantic}: the geographic view highlights the frequent routes and the aggregated POIs with uncertainty encoded as color intensity. The frequently visited POIs in different time are shown in the heatmap.}\label{fig:move_enrich_POI}
\end{figure}
\subsubsection{Mobility Pattern Analysis}
Recent work mainly focuses on analyzing mobility patterns in geospatial movement sequences including traffic trajectories~\cite{krueger2015semantic, poco2015exploring}, cellphone mobility records~\cite{di2016allaboard} and geo-tagged microblogs~\cite{chen2016interactive}.
To capture the geospatial characteristics of movement sequences, researchers often employ geographic maps to visualize the mobility patterns.
%Geospatial movement data are often noisy in real-world applications~\cite{chen2016interactive, di2016allaboard, krueger2015semantic}, which introduces uncertainty in subsequent pattern extraction and visualization.
%Recent work can be categorized based on whether the uncertainty of data is modeled and presented to users.

Lorenzo et al.~\cite{di2016allaboard} present AllBoard, a visual analytics approach for exploring user mobility from cellphone data.
%PrefixSpan~\cite{han2001prefixspan} 
Specifically, they employ a pattern-growth-based algorithm to extract the shared route patterns, which are mapped to the urban transport network to visualize their geographical topology.
Examining the route patterns, users can explore potential directions for optimizing public transport.
Poco et al.~\cite{poco2015exploring} propose a closest path traffic model to calculate the taxi trips and traffic speed from the sparse traffic data.
Using vector field visualizations, the taxi trips along with the traffic speed are visualized in an animated manner, which helps users understand the dynamic traffic pattern of the urban infrastructure.

While those work does not address the inherent uncertainty associated with the data,  modeling and tackling uncertainty with human-in-the-loop can establish a more reliable mobility analysis.
Kruger et al.~\cite{krueger2015semantic} present a visual analytics approach for semantic movement analysis.
They enrich the geospatial movements with POIs obtained from social media.
The POIs are aggregated in the geographical map to indicate the semantics of movements, and the frequent POIs of a focused region are visualized in a heatmap to show the temporal dynamics (Fig.~\ref{fig:move_enrich_POI}).
%and propose a mixed model to address the uncertainty in
As the imprecision of the measurement on time and space can introduce uncertainty in assigning a POI to a geographic position, they propose a mixed model to quantify the uncertainty.
%based on the distance of POI and the number of check-in and log-in records.
For positions with highly uncertain POIs, users can explore their geospatial contexts and determine their POI categories to resolve the uncertainty.
Chen et al.~\cite{chen2016interactive} develop a visual analytics system for exploring Weibo user movement patterns and their semantics.
In particular, they employ Gaussian mixtures to model the uncertainty of movement time interval caused by the sparsity of geo-tagged Weibo data.
The output of Gaussian mixtures are visualized in line charts, where users can interactively steer the model by tuning the number of mixtures and filter the data to reduce the uncertainty.
The filtered data is used to extract reliable movement patterns that are aggregated in a geographic map with the contextual Weibo messages displayed for a semantic exploration.
%to disclose the behaviors of social media users, such as frequent traveling routes.
%aim to tackle the uncertainty of time in the movements extracted from geo-tagged social media.
%``find reliable movement patterns with categorized semantics from geo-tagged Weibo data.''
% movement semantics analysis
%To this end, they employ the Gaussian mixtures to model the uncertainty of time, where users can interactively tune the number of clusters used for fitting Gaussian mixtures.
%The output of Gaussian mixtures are visualized in line charts and a user-driven filtering can be performed to remove unreliable data. 
%aggregated and weibo content as semantics

\begin{figure}[!tb]
  \centering
    \includegraphics[width=0.70\linewidth]{fig/AnomalyDetection_points.pdf}
%     \vspace{-2mm}
%     \caption{EVA~\cite{leite2018eva}: the parallel coordinate plot shows how sub-scores constitute the overall score.}
    \caption{EVA~\cite{leite2018eva}: the parallel coordinate plot shows the contribution of each sub-score to the overall score. The detected anomalous transactions are highlighted.}
%     \vspace{-5mm}
    \label{fig:AnomalyDetection_points}
\end{figure}

==> LaTeX of JOVI-D-18-00101-local/rank.tex <==
\begin{figure*}[!tb]
\centering
    \begin{subfigure}{0.56\textwidth}
          \includegraphics[width=\textwidth]{fig/podium}
    \caption{}\label{fig:podium}
    \end{subfigure}
\centering
    \begin{subfigure}{0.43\textwidth}
          \includegraphics[width=\textwidth]{fig/mutual_ranker}
    \caption{}\label{fig:mutual_ranker}
	\end{subfigure}
    \caption{Example work on interactive information retrieval: (a) Podium~\cite{wall2018podium}: the table view represents each instance as a row and its attributes as columns. Users can drag instances to rank a subset of data; (b) MutualRanker~\cite{liu2016uncertainty}: the composite visualization contains the graph visualization, flow map and glyph,  which visualize ranking results, uncertainty propagation and uncertainty distribution, respectively.}
\end{figure*}
\subsection{Interactive Information Retrieval}
% Interactive ranking is an important visual analytics approach to support decision making~\cite{wall2018podium,pajer2017weightlifter,liang2017photorecomposer}.
We refer to interactive information retrieval as visually ranking or recommending instances for returning relevant information to a query or interactively finding optimal solutions for a decision making.
It has been recently studied in many data-driven applications, such as microblog retrieval~\cite{liu2016uncertainty}, network exploration~\cite{behrisch2017magnostics}, event analysis~\cite{lu2017visual,cho2017crystalball}, document analysis~\cite{park2018conceptvector, wei2010irank} and evolutionary ranking analysis~\cite{lei2016visual}.
Recent work falls into two categories: structured and unstructured information retrieval.
\subsubsection{Structured Information Retrieval}
% \begin{figure}[]\centering
% \includegraphics[width=\linewidth]{fig/podium}
% \caption{}\label{fig:podium}
% \end{figure}
Structured information retrieval is widely used to rank the multi-attribute tabular data to support multi-criteria decision making.
As the ranking results are dependent on the weight of each attribute, recent work mainly focus on exploring the weight space~\cite{pajer2017weightlifter} and interactively learning the weights based on user preferences~\cite{wall2018podium}.

Pajer et al. develop WeightLifter~\cite{pajer2017weightlifter}, a visual analytics system that enables users to visually explore the attribute weight space and gain an understanding of the sensitivity of the ranking to the changes of weights.
%Specifically, they propose two-way and three-way trade-off visualizations to show a slice of weight space.
Their main idea is to visualize slices of weight space and enrich the slices with the projected sensitivity information.
Specifically, they use a vertical axis and barycentric coordinates to show the 1D and 2D slices, respectively.
To visualize the sensitivity of ranking, they segment the weight space based on MCMC sampling and project the segments to the 1D or 2D slices.
By exploring the slices, users can examine the regions where the ranking results are (in)sensitive to changes of weights, and interactively impose constraints on weight space to filter out implausible ranking results.
% Specifically, the sensitivity are calculated using MCMC sampling and users can visually examine the weight regions that the ranking results are insensitive to.
% Furthermore, by allowing users to interactively impose constraints on weight space, the implausible results can be filtered out to save the exploration effort of users. 
%where the selected item is ranked high. 
%thereby perceiving the sensitivity of the ranking to changes of the weights.
%To make it more efficient to support decision making, 
%and inspect the updated ranking sensitivity.

As the data volume and dimensions grow, it may be cognitively hard for humans to specify weights of attributes for ranking the whole data.
Thus, a more plausible way is perhaps to use machine learning models to learn the weights from users' preference. 
Motivated by this, Wall et al. propose Podium~\cite{wall2018podium} to interactively rank the multi-attribute data based on user preference.
They employ Ranking SVM to infer the weight of each attribute from the user preference (i.e., the ranking of a subset of the data).
Particularly, the multi-attribute data are visualized in a table view (Fig.~\ref{fig:podium}), where users can drag the instances to communicate his preference.
%The inferred weights are adopted to rank the whole data using simple Additive Weighting model~\cite{zanakis1998multi}.
%The user can visually perceive the data and interactively ranks the subset of the data. 
%Consequently, the preference of the user is learned by the underlying model and then applied to rank the whole data.
% By doing so, Podium enables a better understanding of the importance of each attribute to user's rankings, and 
% the explicit modeling of user preference avoids requiring users to exactly specify the weights.
% Hence, the human cognitive overhead is greatly reduced.
\subsubsection{Unstructured Information Retrieval}
% \begin{figure}[!tb]\centering
% \includegraphics[width=\linewidth]{fig/mutual_ranker}
% \caption{}\label{fig:mutual_ranker}
% \end{figure}
Interactive information retrieval are recently applied to unstructured data such as texts from social media~\cite{lu2017visual, liu2016uncertainty, cho2017crystalball}, newspaper article comments~\cite{park2018conceptvector}, matrices collections~\cite{behrisch2017magnostics} and photos~\cite{liang2017photorecomposer}.
Due to the unstructured nature of data, characterizing data instances and capturing their relationships are not straightforward and are often specific to data types and applications.
For example, while cosine distance is widely used to measure the similarity between TFIDF features of posts in microblog retrieval~\cite{liu2016uncertainty}, the word embeddings are often employed to characterize words and documents in semantic retrieval applications~\cite{park2018conceptvector}.
% Recent years have also seen the tight integration of human knowledge into refining the relationships between data instances~\cite{liang2017photorecomposer, lu2017visual, park2018conceptvector} and modifying the retrieval results~\cite{liu2016uncertainty}.

Liu et al.~\cite{liu2016uncertainty} propose MutualRanker to interactively retrieve salient data from microblogs and address the uncertainty introduced by the ranking model.
Specifically, they derive the relationships within and between posts, users and hashtags, using the content information of posts as well as their metadata such as hashtag co-occurrences.
Based on the derived relationships, they employ a mutual reinforcement graph model~\cite{duan2012twitter} to rank posts, users and hashtags,
as well as modeling the ranking uncertainty using Poisson mixtures.
The uncertainty of ranking results and its propagation is revealed in a composite visualization (Fig.~\ref{fig:mutual_ranker}), which enables users to refine the ranking results to tackle the uncertainty.
% Upon the user feedback, their approach can locally modify the MRG model using the MC sampling method, thereby yielding a updated ranking result.
% Through interactively refining the MRG model, MutualRanker can produce a high-quality retrieval result and help users gain an understanding of how posts, users and hashtags mutually influence each other, 
% which is beneficial for a more informed decision making.

As semantic similarities between words are important for retrieving documents to a given topic or concept, recent work introduces human-in-the-loop model to interactively learn these semantic similarities.
For example, to retrieve documents relevant to a given topic, Lu et al.~\cite{lu2017visual} propose a user-guided matching model that loops 
human in calculating semantic similarity between words in documents and that in a topic.
Specifically, semantic similarities of words are initially calculated by a knowledge-based method and users can modify the similarities through semantic interaction, i.e., dragging a word from one cluster to another in the force-directed layout.
Consequently, their semantic similarities are adjusted and the relevance of documents are updated.
% Hence, by incorporating human knowledge, the semantic similarities are more consistent to human's mental model and the induced rankings make better sense to humans.
Along the same line, Park et al.~\cite{park2018conceptvector} present ConceptVector, an interactive concept building system for document analysis.
Users specify initial seed keywords to retrieve more relevant words based on the semantic similarities derived from their word embeddings.
The retrieved words are projected in a t-SNE plot, which enables users to visually explore their similarities, label them as relevant or irrelevant.
By modifying related keywords of a concept, users can interactively retrieve the relevant documents for a finer-level analysis.

Cho et al.~\cite{cho2017crystalball} presents CrystalBall for visually analyzing future events extracted from social media.
To identify future events, they propose seven measures to characterize the events and adopt RankSVM~\cite{joachims2002optimizing} to evaluate their quality.
%based on their time-location correlation, informativeness and cohesiveness of the associated tweets.
To present the high quality future events, interactive visualizations are developed to display the ``who, what, when, where'' information, which allows users to visually retrieve the events of interests.

There is some initial work on applying information retrieval on matrix data and photos.
Behrisch et al.~\cite{behrisch2017magnostics} address the task of matrix retrieval based on the feature descriptors of visual patterns such as diagonal blocks.
Specifically, they rank matrices based on the Euclidean distances between their feature descriptors to that of a query matrix.
To select informative feature descriptors, they evaluate each descriptor by the proposed criteria such as pattern discrimination.
Their matrix retrieval approach can be integrated in visual analytics systems to interactively retrieve the matrix and guide the exploration.
Liang et al.~\cite{liang2017photorecomposer} propose PhotoRecomposer, an interactive photo recomposition method based on learning the composition distance metric from user preference.
By ranking the example photos using the learned metric, several reference photos are recommended for recomposing the user photos. 
% Consequently, the instances that are similar to user-preferred ones are ranked higher in the recommendation list, which can save user efforts on refining photo composition.

==> LaTeX of JOVI-D-18-00101-local/task.tex <==
% \begin{table*}\centering
% \caption{A taxonomy of tasks and the recent representative papers. The number of papers is shown in the bracket.}
% \centering\label{table:tasktaxonomy}
% \begin{tabular}{cc}
% \hline
%  \textbf{Task} &  \textbf{Examples} \\
% \hline
% clustering (20)  & ~\cite{kumpf2018visualizing},~\cite{kwon2018clustervision},~\cite{jarema2015comparative},~\cite{wu2017streamexplorer},~\cite{sacha2018somflow},~\cite{andrienko2018clustering},~\cite{onoue2017quasi},~\cite{wu2017making},~\cite{xu2016interactive},~\cite{watanabe2015biclustering},~\cite{rieck2016exploring},~\cite{raidou2016visual},~\cite{zhang2016visualizing},~\cite{badam2017steering},~\cite{wu2015interactive},~\cite{purwantiningsih2016visual},~\cite{wu2017mobiseg},~\cite{heimerl2016citerivers},~\cite{zhao2018bidots},~\cite{sun2016biset}
%  \\
% \hline
% dimensionality reduction (16)  & ~\cite{sacha2017visual},~\cite{wang2018subspace},~\cite{jackle2017pattern},~\cite{xia2018ldsscanner},~\cite{turkay2017designing},~\cite{kwon2017axisketcher},~\cite{pezzotti2017approximated},~\cite{xie2017visual},~\cite{barbosa2016visualizing},~\cite{cheng2016data},~\cite{jackle2016temporal},~\cite{lehmann2016optimal},~\cite{zhou2016dimension},~\cite{wang2017linear},~\cite{liu2015visual},~\cite{pezzotti2016hierarchical}
%  \\
% \hline 
% model understanding (16) & ~\cite{stahnke2016probing},~\cite{liu2016grassmannian},~\cite{wongsuphasawat2018visualizing},~\cite{bilal2018convolutional},~\cite{pezzotti2018deepeyes},~\cite{kahng2018activis},~\cite{rauber2017visualizing},~\cite{liu2017towards},~\cite{liu2018analyzing},~\cite{wang2018ganviz},~\cite{ming2017understanding},~\cite{strobelt2018lstmvis},~\cite{krause2017workflow},~\cite{ren2017squares},~\cite{liu2018visual},~\cite{liu2018visual_we}
%  \\
%  \hline
% classification (11) & ~\cite{el2017nerex},~\cite{verma2017drugpathseeker},~\cite{paiva2015approach},~\cite{tam2017analysis},~\cite{zhang2017quantifying},~\cite{bernard2018comparing},~\cite{muhlbacher2018treepod},~\cite{dou2015demographicvis},~\cite{brooks2015featureinsight},~\cite{yu2015iviztrans},~\cite{rohlig2015supporting}
%  \\
% \hline 
% ranking (8) & ~\cite{liu2016uncertainty},~\cite{behrisch2017magnostics},~\cite{liang2017photorecomposer},~\cite{pajer2017weightlifter},~\cite{lu2017visual},~\cite{wall2018podium},~\cite{cho2017crystalball},~\cite{park2018conceptvector} \\
% \hline
% pattern mining (8) & ~\cite{di2016allaboard},~\cite{poco2015exploring},~\cite{krueger2015semantic},~\cite{chen2016interactive},~\cite{liu2017coreflow},~\cite{liu2017patterns},~\cite{chen2018sequence},~\cite{guo2018eventthread}
%  \\
% \hline
% regression (8) & ~\cite{buchmuller2015visual},~\cite{klemm20163d},~\cite{shao2017interactive},~\cite{zhang2016visual},~\cite{wang2016visual},~\cite{lowe2016visual},~\cite{zhang2015visual},~\cite{bryan2015integrating}
%  \\
% \hline
% anomaly detection (7) & ~\cite{bogl2017cycle},~\cite{cao2016targetvue},~\cite{xu2017vidx},~\cite{leite2018eva},~\cite{lin2017rclens},~\cite{wilkinson2018visualizing},~\cite{cao2018voila}
%  \\
% \hline

% topic modeling (8) & ~\cite{alexander2016task},~\cite{wang2016topicpanorama},~\cite{kim2017topiclens},~\cite{glueck2018phenolines},~\cite{el2018progressive},~\cite{el2016contovi},~\cite{gad2015themedelta},~\cite{thom2015can}
%  \\
% \hline
% \end{tabular}
% \end{table*}
%\begin{table*}[!tbp]\small
\begin{small}
\begin{longtable}{p{3cm} p{3.6cm} p{4.2cm}}
%\vspace{-2mm}
\caption{A taxonomy of tasks and the recent representative papers. \jiangl{The bold texts highlight the tasks that we focus on.} The number of papers is shown in the bracket.}\label{table:tasktaxonomy}\\
\renewcommand\arraystretch{1}
% \begin{tabular}{p{3.48cm} p{4.3cm} p{4cm}}
%\begin{tabular}{p p p}
\textbf{First-level} & \textbf{Second-level} &  \textbf{Examples} \\ \midrule
 \multirow{13}{*}{\makecell[l]{visual cluster analysis (20)}} & \multirow{1}{*}{\makecell[l]{exploratory data analysis (9)}}&\hspace{1sp}\cite{andrienko2018clustering},~\cite{badam2017steering},~\cite{heimerl2016citerivers},~\cite{purwantiningsih2016visual},~\cite{raidou2016visual},~\cite{sacha2018somflow},~\cite{wu2017mobiseg},~\cite{wu2017streamexplorer},~\cite{xu2016interactive}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{comparative \\
 clustering analysis (5)}} & \hspace{1sp}\cite{jarema2015comparative},~\cite{kumpf2018visualizing},~\cite{kwon2018clustervision},~\cite{rieck2016exploring},~\cite{zhang2016visualizing}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{bi-cluster analysis (6)}} & \hspace{1sp}\cite{onoue2017quasi},~\cite{sun2016biset},~\cite{watanabe2015biclustering},~\cite{wu2017making},~\cite{wu2015interactive},~\cite{zhao2018bidots}
\\
\midrule
 \multirow{10}{*}{\makecell[l]{interactive dimensionality \\reduction (16)}} & \multirow{1}{*}{\makecell[l]{ subspace analysis (7)}}&\hspace{1sp}\cite{jackle2017pattern},~\cite{liu2015visual},~\cite{wang2018subspace},~\cite{wang2017linear},~\cite{xia2018ldsscanner},~\cite{xie2017visual},~\cite{zhou2016dimension}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{high-dimensional \\
data exploration (6)}} & \hspace{1sp}\cite{barbosa2016visualizing},~\cite{berger2017cite2vec},~\cite{cheng2016data},~\cite{jackle2016temporal},~\cite{kwon2017axisketcher},~\cite{liu2016grassmannian},~\cite{stahnke2016probing}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{progressive dimensionality\\ reduction (3)}} & \hspace{1sp}\cite{pezzotti2016hierarchical},~\cite{pezzotti2017approximated},~\cite{turkay2017designing}
\\
\midrule
 \multirow{14}{*}{\makecell[l]{interactive model \\analysis (14)}} & \multirow{1}{*}{\makecell[l]{ model understanding (11)}}&\hspace{1sp}\cite{bilal2018convolutional},~\cite{kahng2018activis},~\cite{liu2018analyzing},~\cite{liu2017towards},~\cite{liu2018visual_we},~\cite{ming2017understanding},~\cite{pezzotti2018deepeyes},~\cite{rauber2017visualizing},~\cite{strobelt2018lstmvis},~\cite{wang2018ganviz},~\cite{wongsuphasawat2018visualizing}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{model diagnosis (7)}} & \hspace{1sp}\cite{bilal2018convolutional},~\cite{krause2017workflow},~\cite{liu2018analyzing},~\cite{liu2017towards},~\cite{liu2018visual},~\cite{ren2017squares},~\cite{wang2018ganviz}
\\
\midrule
 \multirow{6}{*}{\makecell[l]{interactive classification (8)}} & \multirow{1}{*}{\makecell[l]{ interactive labeling (4)}}&\hspace{1sp}\cite{bernard2018comparing},~\cite{el2017nerex},~\cite{paiva2015approach},~\cite{yu2015iviztrans}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{interactive \\feature engineering (2)}} & \hspace{1sp}\cite{brooks2015featureinsight},~\cite{dou2015demographicvis}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{parameter spaces analysis (2)}} & \hspace{1sp}\cite{muhlbacher2018treepod},~\cite{rohlig2015supporting}
\\
\midrule
\multirow{6}{*}{\makecell[l]{interactive regression (8)}} & \multirow{1}{*}{\makecell[l]{ interactive \\correlation analysis (5)}}&\hspace{1sp}\cite{klemm20163d},~\cite{shao2017interactive},~\cite{wang2016visual},~\cite{zhang2016visual},~\cite{zhang2015visual}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{interactive \\numerical prediction (3)}} & \hspace{1sp}\cite{bryan2015integrating},~\cite{buchmuller2015visual},~\cite{lowe2016visual}
\\
\midrule
\multirow{5}{*}{\makecell[l]{\textbf{interactive}\\ \textbf{information retrieval (8)}}} & \multirow{1}{*}{\makecell[l]{structured information retrieval (2)}}&\hspace{1sp}\cite{pajer2017weightlifter},~\cite{wall2018podium}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{unstructured information \\retrieval (6)}} & \hspace{1sp}\cite{behrisch2017magnostics},~\cite{cho2017crystalball},~\cite{liang2017photorecomposer},~\cite{liu2016uncertainty},~\cite{lu2017visual},~\cite{park2018conceptvector}
\\
\midrule
\multirow{5}{*}{\makecell[l]{\textbf{visual pattern mining (8)}}} & \multirow{1}{*}{\makecell[l]{exploratory event analysis (4)}}&\hspace{1sp}\cite{chen2018sequence},~\cite{guo2018eventthread},~\cite{liu2017coreflow},~\cite{liu2017patterns}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{mobility pattern analysis (4)}} & \hspace{1sp}\cite{chen2016interactive},~\cite{di2016allaboard},~\cite{krueger2015semantic},
~\cite{poco2015exploring}
\\
\midrule
\multirow{5}{*}{\makecell[l]{\textbf{visual topic analysis (10)}}} 
% & \multirow{1}{*}{\makecell[l]{ topic comparison (6)}}&\hspace{1sp}\cite{alexander2016task},~\cite{el2016contovi},~\cite{gad2015themedelta},~\cite{glueck2018phenolines},~\cite{thom2015can},~\cite{wang2016topicpanorama}
% \\
% \cline {2-3}
%  & \multirow{1}{*}{\makecell[l]{interactive parameter tuning (3)}} & \hspace{1sp}\cite{el2018progressive},~\cite{glueck2018phenolines},~\cite{kim2017topiclens}
% \\
& \multirow{1}{*}{\makecell[l]{flat topic analysis (4)}}&\hspace{1sp}\cite{alexander2016task},~\cite{el2018progressive},~\cite{glueck2018phenolines},~\cite{thom2015can}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{hierarchical topic analysis (4)}} & \hspace{1sp}\cite{kim2017topiclens},~\cite{liu2016online},~\cite{wang2016ideas},~\cite{wang2016topicpanorama}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{topic evolution analysis (3)}} & \hspace{1sp}\cite{el2016contovi},~\cite{gad2015themedelta},~\cite{liu2016online}
 \\
\midrule
\multirow{4}{*}{\makecell[l]{\textbf{interactive} \\ \textbf{anomaly detection (7)}}} & \multirow{1}{*}{\makecell[l]{ anomalous points detection (5)}}&\hspace{1sp}\cite{bogl2017cycle},~\cite{cao2018voila},~\cite{leite2018eva},~\cite{lin2017rclens},~\cite{wilkinson2018visualizing}
\\
\cline {2-3}
 & \multirow{1}{*}{\makecell[l]{anomalous sequences detection (2)}} & \hspace{1sp}\cite{cao2016targetvue},~\cite{xu2017vidx}
\\
\bottomrule
%\end{tabular}
%\end{table*}
\end{longtable}
\end{small}

\section{Analysis on Existing Work}\label{sec:tasks}
In this section, we introduce the recent efforts on IML, with a focus on visual pattern mining, interactive anomaly detection, interactive information retrieval, and visual topic analysis.
\jiangl{We briefly discuss other tasks elaborated by existing IML surveys.}%section \ref{sec:discuss_others}.}
%\input{clustering}
%\input{classify}
%\input{reg}
%\input{high-dim}
\input{pattern}
\input{anomaly}
\input{rank}
\input{topic}
%\input{model}
\input{others}

==> LaTeX of JOVI-D-18-00101-local/topic.tex <==

% \begin{figure}[!tb]\centering
% \includegraphics[width=\linewidth]{fig/topic_panorama}
% \caption{TopicPanorama~\cite{wang2016topicpanorama}: the level-of-detail visualization show a full picture of topics across multiple sources.}\label{fig:topic_panorama}
% \end{figure}
% \begin{figure}[!tb]\centering
% \includegraphics[width=\linewidth]{fig/violin_plots}
% \caption{Violin plots~\cite{el2018progressive} comparatively visualize the weight distribution of each word class from two topic models. }\label{fig:violin_plots}
% \end{figure}
\begin{figure*}[!tb]
\centering
    \begin{subfigure}{0.44\textwidth}
          \includegraphics[width=\textwidth]{fig/topic_panorama}
    \caption{}\label{fig:topic_panorama}
    \end{subfigure}
\centering
    \begin{subfigure}{0.55\textwidth}
          \includegraphics[width=\textwidth]{fig/violin_plots_cropped}
    \caption{}\label{fig:violin_plots}
	\end{subfigure}
    \caption{Example work on visual topic analysis: (a) TopicPanorama~\cite{wang2016topicpanorama}: the graph visualization shows a full picture of topics across multiple sources. The radial icicle plot visualizes the topic hierarchy around the circumference; (b) Violin plots~\cite{el2018progressive} comparatively visualize the weight distribution of each word class from two topic models (encoded by colors).}
\end{figure*}
\subsection{Visual Topic Analysis}
% \begin{figure*}[!tb]\centering
% \includegraphics[width=\linewidth]{fig/topic_modeling_alex_compare}
% \caption{Buddy plots~\cite{alexander2016task}. Each circle represent a document. Given topic models A and B, the position (color) of a document encodes its distance to the reference document in model B (A). 
% The smooth color transition indicates the consistency between A and B, while an abruptive color change indicates their inconsistency. 
% %The color encodes the model-A-induced distance of each document from the reference document. 
% %Blue indicates close in model A while red indicates far in model A.
% }\label{fig:topic_model_compare}
% \end{figure*}
% Suppose A and B are two target topic models to be compared.
% As shown in Fig.~\ref{fig:topic_model_compare}, with each circle representing a document, the position (color) of a document encodes its model-B(A)-induced thematic distance from the reference document.
%The smoothness of color transition can inform users about the consistency between A and B.


% Topic modeling is a popular text-mining technique for discovering latent topics among a collection of documents.
% Recent years has seen the success of visual analytics integrating topic modeling in a vast variety of applications, such as visually summarizing a large corpus~\cite{kim2017topiclens}, understanding texts from multi-sources~\cite{wang2016topicpanorama}, capturing temporal dynamics of the textual data~\cite{gad2015themedelta} and characterizing high-level concepts such as disease subtypes~\cite{glueck2018phenolines}.
% However, due to the unsupervised nature and the underlying mathematical objective not always aligning well to human judgements~\cite{hu2014interactive}, topic modeling sometimes derives poor representation of a topic.
% For example, it may produce a topic represented by semantically incoherent keywords, which does not make sense to humans and thus hampers the thematic understanding of the corpus.
% As humans can detect semantic correlations among topics and words, injecting human knowledge into topic models(i.e., interactive topic modeling) is beneficial to finding salient semantic patterns from textual data.
% Surveying the relevant literatures, we find there are two main challenges of performing an effective interactive topic modeling.
% First, since topic modeling is usually regarded as a black box~\cite{el2018progressive}, we need to deeply understand the model so as to diagonose and refine it.
% Second, it is a still an open question on how to sensibly incorporating human knowledge and then adjust the topic models accordingly.
% As a result, below we introduce two recent work that strive to provide a better understanding of topic models and steer the topic models by integrating human knowledge.

% The very first work is presented by Alexander et al.~\cite{alexander2016task}. 
% They argue that explicitly comparing different topic models is helpful to a nuanced understanding 
% of the models.
% Along this line, they identify three main tasks for model comparison, i.e., topic alignment, distance comparison, timeline comparison.
% The goal of the tasks is to promote the understanding of the topic model from distinct perspectives.
% Below we briefly introduce each task and the employed visualization techniques. 
% We suppose two topic models A and B are the target models to compare for all the three tasks.

% For topic alignment task, they calculate similarities between each topic derived by A and that by B, 
% then they visualize the similarities using an enriched parallel-coordinate-like plot.
% Uses can browse the plots to spot two kinds of topic matching, i.e., bi-directional match, one-directional match.
% For bi-directional matched topics, it is likely to be a semantically salient topic so users can explore the associated words of documents to understand the topic semantics.
% For one-directional match, it may indicate one model splits or merges topics from the other model, because the match is directional.
% Users can thus drill in to the underlying words and documents to confirm the hypothesis and gain an understanding of why the split/merge happens.

% For the distance comparison task, they propose a novel visualization design named buddy plots, for inspecting consistency between topic models.
% As shown in Fig.~\ref{fig:topic_model_compare}, given a reference document (Hamlet in this case), 
% the rest of the documents (represented as a circle) are positioned along a line.
% The position (color) of the document encodes its model-B(A)-induced thematic distance from the reference document.
% Thus, if model A aligns well to model B, users can perceive a smooth color transition from blue to red, 
% else, the abruptive color change could easily be captured by users, which indicates model A and model B produce noticeably inconsistent results.
% Hence, buddy plot highlight the difference of two topic modeling results and enable an effective visual comparison of model consistency.

% For the timeline comparison task, they use the similar visualization to ThemeRiver~\cite{havre2002themeriver} for displaying the trends of topic distribiutions over time.
% Users can compare the thematic trends derived from two models and consequently find informative patterns that are valuable for understanding the model behaviors.
% For example, if model A consistently produce trends that are merged by model B, then it is possible that the topic number of model A is too large to fit the corpus.

% In spite of the effectiveness on comparative analysis, 
% their methods are limited to inspecting model outputs and no further actions (such as interactions for modifying topic number) are taken for
% tuning the unsatisfactory model based upon the gleaned insights.

% In light of this, El-Assady et al.~\cite{el2018progressive} presents an interactive visualization that go beyond pairwise topic model comparison.
% Their goal is to address the interpretability and adaptability (how adaptable the model is upon user feedback) of topic models.
% To this end, they propose a visual analytics framework where the topic models are progressively optimized in a user-driven manner.
% Specifically, their framework comprises of four views designed for their respective analysis task.

% The first view is aimed to provide an overview of topic matching results.
% It visualizes keywords of derived topics from two models and the matching degree of two models.
% Users can explore the overview and select a pair of topics to drill in to the next view. 
% The second view is tailored to topic summarization task.
% The keywords of the selected topic along with its relevance to the topic are visualized.
% The ten most relevant sentences from the corpus are also presented, so user can capture the 
% semantics of the topic by browsing the keywords and inspecting the supporting sentences.
% Besides, the mirrored bar charts in the middle of the view shows the documents that contains the particular topic.
% Users can thus understand the distribution of the topic prevalence over documents.
% By clicking the mirrored bar chart, users can move on to the next view to study parameter distribution.
% The parameter distribution view visualizes the parameter (weight of word class) distribution over the documents.
% Users can compare the parameter distributions from two models through the violin-style plots and then select the specific document to inspect further in the next view.
% The last view allows document relevance feedback.
% In this visualization, users are presented with the texts of the selected document along with the topics derived by two models respectively.
% Inspecting the detailed text information of the document, users would prefer the topic learned by one model over the other, so he could adjust the decision-slider to one side to communicate his preference.
% Besides, users are also permitted to directly express his preference regarding the keywords using this visualization.
% The preference of the user are then used to adjust the weights of the affected keywords, i.e., the keyword from favored topic model is boosted while the keyword from
% rejected topic model is penalized.
% The topic models are then recomputed by integrating the updated weights.

% Overall, the four-stage layered analysis indeed foster a better understanding of topic modeling.
% Empirical evidence also showcases the effectiveness of the human-in-the-loop learning paradigm.
% However, while we believe this paper serves as an entry point to addressing interactive topic modeling, 
% it could be extended to go deeper into the topic models, such as visualizing parameter inference process, 
% which is critical to explaining why a particular topic assigns high probabilities to certain keywords.
% Topic modeling is a popular text-mining technique for discovering latent topics inside a document collection.
% Each topic is represented by a set of keywords derived from the documents and each keyword has a probability value to indicate its relevance to that topic.
% Visual analytics approaches for topic modeling are recently proposed for handling several real-world tasks, such as analyzing topics from multiple sources~\cite{wang2016topicpanorama} and characterizing disease subtypes from clinical  data~\cite{glueck2018phenolines}.
Visual topic analysis is a popular visual analytics technique for understanding and analyzing latent topics inside a document collection.
Each topic is represented by a set of keywords derived from the documents and each keyword has a probability value to indicate its relevance to that topic.
Recent efforts on visual topic analysis focus on efficiently handling  real-world tasks such as analyzing topics from multiple sources~\cite{jiang2016text,wang2016topicpanorama}, characterizing disease subtypes from clinical  data~\cite{glueck2018phenolines} and review analysis~\cite{xu2018vaut}.
% The textual data is often collected from multiple sources, such as news article, social media messages and scientific publications.
%capturing temporal dynamics of the textual data~\cite{gad2015themedelta} exploring a large corpus~\cite{kim2017topiclens}
%In this section, we summarize these work from two perspectives: topic comparison and interactive parameter tuning.
Following the task taxonomy of a recent text visualization survey~\cite{liu2018bridging}, we summarize the work pertinent to visual topic analysis from three perspectives: flat topic analysis, hierarchical topic analysis and topic evolution analysis.
\subsubsection{Flat Topic Analysis}
Recent work on analyzing topics organized in a flat structure mainly addresses topic comparison task.
They can be classified into two categories: within-model topic comparison, between-model topic comparison.

The within-model topic comparison can disclose how topics are related to each other, which facilitates users to examine semantic differences of topics and make a more informed optimization~\cite{glueck2018phenolines}.
Recent works mainly display the juxtaposition of topic visualizations for comparing different topics.
For example,  Glueck et al.~\cite{glueck2018phenolines} presents PhenoLines, a visual analysis tool for disease subtype analysis based on topic modeling.
They apply LDA~\cite{blei2003latent} on electronic health care records, where patients, phenotypes and disease subtypes are modeled as documents, words and topics, respectively.
Mapping the words to a phenotype ontology, each topic is visualized in a sunburst diagram.
They juxtapose the sunburst diagrams of different topics to enable a between-topic comparison.
Some actionable insights are derived from the comparison. 
For example, they show that a prior distribution that emphasize the words that frequently occur in the data, can better differentiate topics than a non-informative Dirichlet prior.
Along the same line, Thom et al.~\cite{thom2015can} juxtapose the word clouds that visualize the keywords of topics, to enable a semantic comparison between topics for situational awareness analysis on social media.

The between-model topic comparison can help validate the gained insights~\cite{alexander2016task}, select models and tune their parameters~\cite{alexander2016task, el2018progressive}.
Alexander and Gleicher~\cite{alexander2016task} propose a task-driven approach for between-model topic comparison.
They characterized three main specific comparison tasks: topic alignment, distance comparison and timeline comparison.
To tackle these tasks, they apply existing visualization techniques such as heatmaps and parallel coordinates, as well as a novel ``buddy plot'' for examining the consistency of document distances derived from two topic models.
El-Assady et al.~\cite{el2018progressive} propose a progressive visual analytics approach to optimize weights of word class (e.g., nouns).
They present comparative visualizations of two topic modeling results for users to examine topic matching, explore topic semantics, understand distributions of weights over documents, and inspect the texts of documents for communicating his or her preference of one topic model.
In particular, they propose ``violin plots'' to enhance the comparison between weight distributions from two topic models (Fig.~\ref{fig:violin_plots}).
The preference of the user is used to adjust the weights of the affected keywords, i.e., the weight of keywords from the favored topic model is increased while the keyword from the other model is penalized.
\subsubsection{Hierarchical Topic Analysis}
Organizing the topics into a hierarchy can alleviate the visual clutter problem caused by the massive amount of topics, and provide richer information to reveal the latent relationships between topics~
\cite{dou2016topic, wang2016topicpanorama}.
Recently, researchers develop level-of-detail visualizations to present the hierarchical topic relationships to users,  allow them to dive into the details and refine the topic hierarchy.

Wang et al.~\cite{wang2016topicpanorama} present TopicPanorama, a visual analytics system for understanding the topics across multiple sources.
They extract topic graphs from multiple sources using correlated topic models~\cite{chen2013scalable}, then match them using a consistent graph matching algorithm and cluster them into the topic hierarchies by a constraint-based algorithm.
The matching results are presented in a graph visualization with
topic hierarchies displayed by a radial icicle plot around the circumference (Fig.~\ref{fig:topic_panorama}), which enables users to find common topics discussed across multiple sources and distinctive ones covered in each individual source.
By incorporating an online metric learning algorithm, users are allowed to interactively modify the graph matching results based on their knowledge.
There is some recent work on refining topic hierarchy based on altering the cluster number.
Kim et al.~\cite{kim2017topiclens} propose a nonnegative-matrix-decomposition-based topic model that can build the topic hierarchy in a user-driven manner.
The initial topic hierarchy is learned by the topic model with a predefined cluster number.
Users can refine the initial hierarchy by overlaying a lens on a region of interest in the t-SNE plot of documents, to trigger an increase of the cluster number.
Consequently, the nodes of the hierarchy that accommodate the documents in the focused region, are split into more clusters, which reveals a finer-level structure of topics.
\subsubsection{Topic Evolution Analysis}
Analysis of topic evolution is important to understanding dynamic patterns in time-varying documents~\cite{liu2014survey, liu2016online}.
For example, Gad et al.~\cite{gad2015themedelta} quantify the temporal shift of topics by measuring the keyword overlap between topics.
Based on the shift of topics, they propose a temporal segmentation algorithm to detect the time step where the topic distributions are significantly changed.
By visualizing the common keywords across time segments using trendlines, the temporal dynamics of topics such as merging or splitting are disclosed.
El-Assady et al.~\cite{el2016contovi} develop ConToVi, a visual analytics system for exploring thematic dynamics of speaker utterances in multi-party conversation.
Specifically, they employ a hierarchical topic model to extract the topic structures and the speaker-topic relationships, which are visualized in a topic-space radial layout.
Comparing the positions of speakers in the topic-space, users can explore the thematic focuses of speakers.
By animating the radial layout, users can track the topic shift indicated by the transition of speaker positions.
%--------------------------------split line--------------------------------------------
% \subsubsection{Topic Comparison}
% Recent work on comparative analysis of topics can be classified into three categories: comparing different topics within a single model, comparing topics from different models, and comparing topics from multiple sources.

% To compare different topics within a single model, Glueck et al.~\cite{glueck2018phenolines} presents PhenoLines.
% They apply LDA~\cite{blei2003latent} on electronic health care data, where patients, phenotypes and disease subtypes are modeled as documents, words and topics, respectively.
% Mapping the words to a hierarchical phenotype ontology, each topic is visualized separately in a sunburst diagram.
% By exploring the juxtaposition of the sunburst diagrams of different topics, users can make a between-topic comparison. 
% Similarly, Thom et al.~\cite{thom2015can} use LDA to extract topics from Twitter data, visualize each topic using word cloud, and juxtapose word clouds for a semantic comparison.
% Comparison between topics in different time steps can reveal the temporal evolution of topics.
% For example, Gad et al.~\cite{gad2015themedelta} quantify the temporal shift of topics by measuring the keyword overlap between topics.
% Based on the shift of topics, they propose a temporal segmentation algorithm to detect the time step where the topic distributions are significantly changed.
% By visualizing the common keywords across time segments using trendlines, the temporal dynamics of topics such as merging or splitting are disclosed.
% El-Assady et al.~\cite{el2016contovi} develop ConToVi, a visual analytics system for exploring thematic dynamics of speaker utterances in multi-party conversation.
% Specifically, they employ a hierarchical topic model to extract the topic structures and the speaker-topic relationships, which are visualized in a topic-space radial layout.
% Comparing the positions of speakers in the topic-space, users can explore the thematic focuses of speakers.
% By animating the radial layout, users can analyze the topic shift indicated by the transition of speaker positions.

% To compare topics from different models, Alexander and Gleicher~\cite{alexander2016task} propose a task-driven approach.
% They characterized three main comparison tasks: topic alignment, distance comparison and timeline comparison.
% To tackle these tasks, they apply existing visualization techniques such as heatmaps and ThemeRiver~\cite{havre2002themeriver}, as well as a novel ``buddy plot'' for examining the consistency of document distances derived from two topic models. 
% %(Fig.~\ref{fig:topic_model_compare}).


% For comparing topics from multiple sources, Wang et al.~\cite{wang2016topicpanorama} presents TopicPanorama.
% The topic graphs from multiple sources of textual corpus are extracted by correlated topic models~\cite{chen2013scalable} and matched using a consistent graph matching algorithm.
% The matching results are presented in a level-of-detail visualization (Fig.~\ref{fig:topic_panorama}), which enables users to find common topics discussed across multiple sources and distinctive ones covered in each individual source.
% By incorporating online metric learning algorithm, users are allowed to interactively modify the graph matching results based on their knowledge.
% % Additionally, to capture potential user requirements, users are allowed to interactively modify the graph matching results.
% \subsubsection{Interactive Parameter Tuning}
% Recent work mainly focus on tuning the weight of words~\cite{el2018progressive}, topic priors~\cite{glueck2018phenolines} and cluster number~\cite{kim2017topiclens} for interactively refining topic models.

% El-Assady et al.~\cite{el2018progressive} propose a progressive visual analytics approach to optimize weights of word class (e.g, nouns).
% They present comparative visualizations of two topic modeling results for users to examine topic matching, explore topic semantics, understand distributions of weights over documents, and inspect the texts of documents for communicating his or her preference of one topic model.
% % Specifically, they provide comparative visualizations of two topic modeling results, where keywords and their supporting sentences are displayed to capture the semantics of the topics.
% In particular, they propose ``violin plots'' to enhance the comparison between weight distributions from two topic models (Fig.~\ref{fig:violin_plots}).
% % Inspecting the texts of a document, users can select a preferred topic model.
% The preference of the user is used to adjust the weights of the affected keywords, i.e., the weight of keywords from the favored topic model is increased while the keyword from the other is penalized.
% %The topic models are then recomputed by integrating the updated weights.

% Besides tuning the weights of words, changing the prior distribution of topic is also investigated by researchers.
% For example, Glueck et al.~\cite{glueck2018phenolines} show that a prior distribution that emphasize the words that frequently occur in the data, can better differentiate topics than a non-informative Dirichlet prior.

% There is some recent work on refining topic models based on altering the cluster number.
% Kim et al.~\cite{kim2017topiclens} propose a nonnegative-matrix-decomposition-based topic model that can build the topic hierarchy in a user-driven manner.
% The initial topic hierarchy is learned by the topic model with a predefined cluster number.
% Users can refine the initial hierarchy by overlaying a lens on a region of interest in the t-SNE plot of documents, to trigger an increase of the cluster number.
% Consequently, the nodes of the hierarchy that accommodate the documents in the focused region, are split into more clusters, which reveals a finer-level structure of topics.


